PriCL: Creating a Precedent A Framework for Reasoning about Privacy Case Law

We introduce PriCL: the first framework for expressing and automatically reasoning about privacy case law by means of precedent. PriCL is parametric in an underlying logic for expressing world properties, and provides support for court decisions, their justification, the circumstances in which the justification applies as well as court hierarchies. Moreover, the framework offers a tight connection between privacy case law and the notion of norms that underlies existing rule-based privacy research. In terms of automation, we identify the major reasoning tasks for privacy cases such as deducing legal permissions or extracting norms. For solving these tasks, we provide generic algorithms that have particularly efficient realizations within an expressive underlying logic. Finally, we derive a definition of deducibility based on legal concepts and subsequently propose an equivalent characterization in terms of logic satisfiability.

==> prelim.tex <==



The framework has to be capable of reasoning about
adjudication. Consequently, we require the possibility to use tools
based on decidable algorithms. For this purpose we introduce the
description logic ``attributive concept language with complements'',
short $\ALC$, in this section. The reader who is familier with $\ALC$
might skip this section. Our description of $\ALC$ follows the work of
Baader, Horrocks and Sattler~\cite{BaHS07a}.


\begin{definition}[$\ALC$ syntax]
  Let $N_C$ be a set of \emph{concept names} and $N_R$ be a set of
  \emph{role names}. The set of \emph{$\ALC$-concept descriptions} is
  the smalles set such that
\begin{enumerate}
\item $\top,\bot$ and every concept name $A\in N_C$ is an $\ALC$-concept,
\item if $C$ and $D$ are $\ALC$-concepts and $r\in N_R$, then $C\sqcap
  D$, $C\sqcup D$, $\lnot C$, $\forall r.C$, and $\exists r.C$ are
  $\ALC$-concepts.
\end{enumerate}

A \emph{general concept inclusion (GCI)} is of the form $C\sqsubseteq D$, where
$C,D$ are $\ALC$-concepts. A finite set of GCIs is called a \emph{TBox}.
%
An \emph{assertional axiom} is of the form $x : C$ or $(x,y) : r$, where $C$ is
am $\ALC$-concept, $r$ is an $\ALC$-role, and $x$ and $y$ are individual
names. A finite set of assertional axioms is called an \emph{ABox}.

A \emph{knowledge base (KB)} is a pair $(\mathcal{T},\mathcal{A})$,
where $\mathcal{T}$ is a TBox and $\mathcal{A}$ is an ABox.
\end{definition}

The semantic of $\ALC$ is intuitively based on interpretation models
which is a set of sets, i.e., every concept and role relate to sets and
the operations defined are defined by the naturally corresponding set
operations. Validity is defined by the requirement that something holds
for every interpretation and satisfiability the existence of an
interpretation.

Now, we consider the operations for which we are interested in
reasoning, i.e., deciding whether these are valid or satisfiable for a
specific knowledge bases. Here, the following three tasks are of
interest: is a knowledge base $\KB$ consistent? Does concept $C$ subsume
concept $D$ ($D\sqsubseteq C$)? Is an individual $a$ an instance of a
concept $C$ ($a\in C$)?  These questions are decidable, however, they
are $\exptime$-complete. For further details on $\ALC$, we refer to
\cite{BaHS07a}.


Finally, we define some syntactic sugar which we will use later in our
framework.

\begin{definition}[Syntactic sugar]
  For two knowledge bases $\KB_A = (\mathcal{T}_A,\mathcal{A}_A)$ and
  $\KB_B = (\mathcal{T}_B,\mathcal{A}_B)$, we define $\KB_A\wedge\KB_B
  := (\mathcal{T}_A\cup\mathcal{T}_B,\mathcal{A}_A\cup\mathcal{A}_B)$.
%
  In addition, we will use a propositional logic (with standard
  semantics) on top of the queries described above.
\end{definition}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> proofs/case_comp_lemma.tex <==
\
\begin{proof}

  First consider the case $C^F_{\sub(n)} := (n,F,\sub(n),\crt)$.  Since
  all leaf nodes of $\sub(n)$ are also leaves of $\prTree$ it follows
  that $\KB_W\wedge F\models\req(n)$, which ensures the leaf node
  property of consistency. In addition, the inner nodes do not change
  and $\KB_W\wedge F\not\models\bot$ together with $\KB_W\wedge
  F\models\req(n)$ implies that $\KB_W\wedge F\wedge\req(n)
  \not\models\bot$.  Hence, the reasoning steps also hold for $\sub(n)$
  and $C^F_{\sub(n)}$ is a consistent case.

  Now consider $C^F_{\compress(n)} = (n,F,\compress(n),\crt)$. The
  argumentation for the leaf nodes is the same as for $C^F_{\sub(n)}$,
  however, there are no inner nodes except the root. 

  The rest of the proof follows by the fact that the children nodes
  imply the underlying inner node. This allows to move children from a
  node $n$ to it's parent node maintainig the consistency properties.
%   \TODOJ{Um, if I understand well, the rest of the proof is about
%     arguing that ``(*) given each inner node is a formula implied by
%     its children, it follows that the leaves imply the root''? If so,
%     I strongly suggest to omit the proof. In all circumstances I can
%     imagine, (*) is a property that every reader would consider as
%     obviously true.}
%
%   We prove the rest by induction on the longest path to a leaf node from
%   $n$. The base case, i.e., $n$ is leaf node. Then $C^F_{\compress(n)} =
%   C^F_{\sub(n)}$, so the statement follows from the fact that
%   $C^F_{\sub(n)}$ is consistent.
%
%   Next, we consider the induction step, i.e., for all nodes having a
%   shorter distance to the leaves than $n$ the statement has been shown,
%   we need to show it for node $n$.
%
%   For all children nodes $n_1,\ldots,n_k$ of $n$ which are inner nodes,
%   we can apply the induction hypothesis since $\KB_W\wedge
%   F\models\req(n)$ implies $\KB_W\wedge F\models\req(n_r)$ for all
%   $r\in\{1,\ldots,k\}$. Therefore we get consistent cases
%   $C^F_{\compress(n_1)},\ldots,C^F_{\compress(n_k)}$ which only contain
%   the inner node $n_i$ and leaf nodes.  Let $l_1,\ldots,l_j$ be the
%   children of $n$ which are leaves.  We can replace the children
%   $n_1,\ldots,n_k$ of $n$ by the compressed proof trees since these are
%   consistent and the consistency condition for $n$, i.e.,
%
%   \[ \bigwedge_{1\leq r\leq k}n_r\wedge\bigwedge_{1\leq i \leq j}
%   l_i\models n \]
%
%   is still fulfilled. Thus the constructed case is consistent.%  Let
%   % $l_{i+1},\ldots,l_j$ be the leaves annotated by $\labAxiom$. By
%   % consistency, it follows that $\KB_W\wedge\caseDesc\models l_{r}$ for
%   % $r\in\{i+1,\ldots,j\}$. Thus for $L:=\bigwedge_{i<r\leq j} l_r$, it
%   % holds that $\KB_W\wedge\caseDesc\models L$ and consequently
%   % $\KB_W\wedge\caseDesc\wedge\{n_1,\ldots,n_k,l_1,\ldots,l_i\}\models
%   % n$. Therefore, we can remove the nodes labeled by $\labAxiom$ and
%   % maintain consistency for the constructed case.
%   %
%   It is easy to see that two neighboring inner nodes $n_a,n_b$ can be
%   combined to a node $n_a\wedge n_b$ by adding all children of $n_a$ and
%   all of $n_b$ to that node. Doing so, we achieve a case that has $n$ as
%   a node and one inner chlid $n_1$ which is still consistent. 
% %
%   We can remove this inner node $n_1$ if we add it's children to $n$
%   directly. Since then that children imply $n_1$ and $n_1$, together
%   with the neighboring leaves, implies $n$.
%
%   Summarized, we constructed from $C^F_{\sub(n)}$, which is a consistent
%   case, the case $C^F_{\compress(n)}$ by applying only steps that preserve
%   the property of consistency, i.e., $C^F_{\compress(n)}$ is consistent.
%
\end{proof}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../main"
%%% End: 


==> proofs/conflictProofBot.tex <==

\begin{proof}
  Let $\mathcal{N}$ be the set of nodes that prove that $\mathcal{C}$ is
  in conflict. 
%  
  Define a proof tree $\prTree$ as a tree with $\mathcal{N}$ leaf nodes
  and a root node annotated by $\bot$. For every $n\in\mathcal{N}$ there
  is a case $C_n$ such that $n$ is in $C$'s proof tree. Thus, we add a
  leaf containing $n$ annotated by $\labCase(C_n)$ for every $n$. We
  also add a leaf node $\KB_W$ labeled with $\labAxiom$. Let
  $C:=(\bot,\top,\prTree,\crt)$ for an arbitrary $\crt\in\courtSet$.
%
  The proof tree is consistent since $\KB_W\wedge\top\models\KB_W$
  and $\KB_W\wedge\bigwedge_{n\in\mathcal{N}}\req(n)\models\bot$.
%
  % The case $C$ also references correctly (up to the fact that
  % $\refer(C)$ is in conflict) since $(n,\req(n),\sub(n),\crt)$ is
  % consistent for consistent $C_n$.
\end{proof}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../main"
%%% End: 


==> proofs/consistencyPreventsBot.tex <==

\begin{proof}
  The property (2) follows immediately from (1) since deducability of
  $\bot$ implies that $\DB\cup C$ is consistent for some $C$ that has
  root node $\bot$.
%
  In the following, we prove (1). Assume $\bot\in C$ and $C$ is
  consistent.  Let $n$ be the node that contains $\bot$. By consistency
  of $C$'s proof tree, it follows that
  $\KB_W\wedge\caseDesc\wedge\req(n)\models n$ therefore. For the set
  $\mathcal{N}:=\{n\}$ it follows that $\{C\}$ is in conflict
  because. This contradicts that $C$ is consistent.
%
%  
  % Assume the predicate $\bot$ is deducable. % Then there
  % % is a case $C$ such that $\DB\cup\{C\}$ is consistent and $C$ proves
  % % $\bot$ without using a $\labDec$ node.
  % By Theorem~\ref{lemma:allFollowsFromDecisions} we know that there is a
  % set $\mathcal{D}$ of decisions such that \[
  % \KB_W\wedge\bigwedge_{f\in\mathcal{D}} f \wedge \caseDesc \models
  % \bot \] Since $\mathcal{D}$ contains only finitely many elements, a
  % minimal $\mathcal{D}$ exists, and hence, we assume $\mathcal{D}$ to be
  % minimal.  Therefore, for an arbitrary $\bar f\in\mathcal{D}$, it holds
  % that
  % $\KB_W\wedge\caseDesc\wedge\bigwedge_{f\in\mathcal{D}\backslash\{\bar
  %   f\}}f\models\lnot \bar f$. Let $C_{\bar f}$ be the case containing
  % decision node $\bar f$. The cases $C$ and $C_{\bar f}$ are
  % conflicting. This is the case since $C$ references correctly and is
  % consistent, and therefore $\KB_W\wedge\caseDesc\models \req(n_{\bar
  %   f})$ where $n_{\bar f}$ is the node corresponding to $\bar f$ in
  % $C_{\bar f}$.
%
  % In fact, the case $C$ introduces at least as many conflicts as the
  % size of $\mathcal{D}$.
%
  % Without loss of generality, we can assume that $C$ is compressed
  % (lemma~\ref{lemma:case:compression}).  The root contains $\bot$. Since
  % $C$ is consistent, it holds that
  % $\KB_W\wedge\{\concl_1,\ldots,\concl_k\}\models\bot$. Since $C$ does
  % neither contain $\labDec$ nor $\labAxiom$, all conclusions $\concl_i$
  % are based on case references and the case description. Let
  % $\mathcal{D}$ be the $\concl_i$ that are based on leaves labeled by
  % $\labDesc$ and $\mathcal{R}$ the ones obtained by case references.
\end{proof}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../main"
%%% End: 


==> proofs/followsFromDecisions.tex <==

\begin{proof}

  The proof consists of two steps: first we transform $\DB$ into a
  different $\DB$, without changeing the properties of referencial
  consistency and case-wise consistency, that still contains the same set
  of leaf nodes. Therefore it suffices to show the theorem for this
  $\DB$ set. In the second step of the proof, we show the theorem's
  claim by induction on the order $\leref$.


  \paragraph{$\DB$ transformation}
  The goal of the theorem is to show that the court decision only
  depends on other decisions or in other words, that the $\labCase$
  leaves can be replaced by decision nodes in the
  argumentation. Therefore, we need to prepare the database by using the
  compression lemma on nodes that are referenced by $\labCase$
  leaves. So, for every case $C=(\confPred,\caseDesc,\prTree,\crt)$ we
  do the following operation on the case law database:
  \begin{itemize}
\item Let $N$ be the set of nodes $n\in\prTree$ such that $\labCase(D)$ is a leaf
  node of $C$.
\item For every $n\in N$, let $E(C,n):=C^{\caseDesc}_{\compress(n)}$ be
  the case that is constructed when compressing $D$ to the node $n$
  using the case description $\caseDesc$ of $C$. In particular, $E(C,n)$
  is a consistent case since $\KB_W\wedge\caseDesc\models\req(n)$ by
  referential consistency of $\DB$ and consistency of $C$ implies that
  $\KB_W\wedge\caseDesc\not\models\bot$. Hence, applying
  lemma~\ref{lemma:case:compression} gives that $E(C,n)$ is consistent.
  In addition, $E(C,n)$ references correctly w.r.t. $\DB$ since $D$ does
  so. Therefore we can add $E(C,n)$ to $\DB$ maintaining referential and
  case-wise consistency.%  \TODOJ{see above: I don't see why the claim of
    % the theorem woukd require us to do that. it seems we are proving a
    % different (stronger) claim here.}
\item We can replace $C$ in $\DB$ by a case $C'$ that references
  $E(C,n)$ instead of $D$. This does not change the case wise
  consistency, since none of the formulas in $C$ changed, and
  referential consistency is preserved since $\refer{C}$ did not change
  and since $E(C,n)$ is the subcase that needs to be consistent for
  referential consistency.
  \end{itemize}
  
  Using this transformation ensures that $E(C,n)\leref C$ and we can
  assume that every reference ends in a tree that consists of the root
  and children leaf nodes without further inner nodes. The claimed
  property can now be easily shown using induction on $\leref$ applying
  the induction hypothesis on $E(C,n)$ for $C$. The base case follows
  since there are no $\labCase$ leaves there.
%
%   \paragraph{Proof of the claimed property} We prove the theorem on the
%   transformed $\DB$ by induction on $\leref$: 
%
% \begin{itemize}
% \item \textbf{Base case:} $C$ is minimal w.r.t. $\leref$,i.e.,
%   $\lnot\exists D\in\DB:D\leref C$.
%
%   That means that no leaf of $C$ is annotated by $\labCase(D)$ for any
%   $D$ since otherwise $D\leref C$ would hold, i.e., $C$ would not be
%   minimal. Thus all leaves are annotated by $\labDec$ or $\labAxiom$.
%
%   If $p$ is a leaf node, we take $\mathcal{D}$ as that leaf node and
%   nothing has to be shown. Thus assume that $p$ is an inner node of the
%   proof tree.  By the case compression
%   lemma~\ref{lemma:case:compression} the case
%   $C^{\caseDesc}_{\compress(n)}$ is consistent. For the set
%   $\mathcal{D}$ defined as the set of formulas representing the decision
%   leaves of $C^{\caseDesc}_{\compress(n)}$ it holds that
%   \[ \KB_W \wedge \caseDesc \wedge \bigwedge_{f\in\mathcal{D}} f \models
%   p \] by consistency since $C$ does not have $\labCase$ leaves.
%
% \item \textbf{Induction step:} The statement holds for all $D\leref
%   C$. We show that it also holds for $C$.
%
%   First consider $p$ to be a leaf node of the proof tree. If $p$ is
%   labeled by $\labDec$ or $\labAxiom$ nothing is to show as in the base
%   case. If $p$ is labeled by $\labCase(D)$, then $E(C,p)\leref C$ holds
%   and the statemet follows by the induction hypothesis.  So, consider
%   $p$ to be an inner node of the proof tree.
%
%   By the compression lemma, it follows that
%   $C^{\caseDesc}_{\compress(p)}$ is consistent. Let $n_1,\ldots,n_k$ be
%   the leaves of $C^{\caseDesc}_{\compress(p)}$ that are annotated by
%   $\labCase(D_i)$ for some case $D_i$ (by referencial consistency these
%   cases exist). In particular, the case $E(C,n_i)\leref C$ and we can
%   apply the induction hypothesis and get sets
%   $\mathcal{D}_1,\ldots,\mathcal{D}_k$ such that
%   $\bigwedge_{f\in\mathcal{D}_i} f\wedge \KB_W\wedge\caseDesc\models
%   n_i$. Here, it is important that the cases $E(C,n_i)$ all have the
%   same case description $\caseDesc$ as $C$. Let $d_1,\ldots,d_r$ be the
%   leaves of $C^{\caseDesc}_{\compress(p)}$ labeled by $\labDec$ and
%   $g_1,\ldots,g_s$ be the leaves labeld by $\labAxiom$. Summarized we
%   get the following statements:
% %
%   \begin{align*}
%     \bigwedge_{1\leq i\leq r} d_i \wedge \bigwedge_{1\leq
%       i\leq k} n_i \wedge \bigwedge_{1\leq j\leq s} g_j&\models p\\
%     \forall i: \bigwedge_{f\in\mathcal{D}_i} f\wedge \KB_W \wedge
%     \caseDesc & \models n_i\\
%     \forall j: \KB_W\wedge\caseDesc&\models g_j
%   \end{align*}
% %
%   Defining $\mathcal{D}' := \bigcup_{1\leq i\leq k} \mathcal{D}_i$, we
%   can derive the following:
% %
%   \[ \KB_W\wedge\caseDesc\bigwedge_{f\in\mathcal{D}'} f \models
%   \bigwedge_{1\leq i\leq k} n_i \]
% %
%   Thus the set $\mathcal{D}:=\mathcal{D}'\cup\{d_i\mid 1\leq i\leq r\}$
%   fulfills the properties stated in the lemma.
% \end{itemize}
\end{proof}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../main"
%%% End: 

